Exploring and machine learning structural instabilities in 2D materials

We address the problem of predicting the zero-temperature dynamical stability (DS) of a periodic crystal without computing its full phonon band structure. Here we report the evidence that DS can be inferred with good reliability from the phonon frequencies at the center and boundary of the Brillouin zone (BZ). This analysis represents a validation of the DS test employed by the Computational 2D Materials Database (C2DB). For 137 dynamically unstable 2D crystals, we displace the atoms along an unstable mode and relax the structure. This procedure yields a dynamically stable crystal in 49 cases. The elementary properties of these new structures are characterised using the C2DB workflow, and it is found that their properties can differ significantly from those of the original unstable crystals, e.g. band gaps are opened by 0.3 eV on average. All the crystal structures and properties are available in the C2DB. Finally, we train a classification model on the DS data for 3295 2D materials in the C2DB using a representation encoding the electronic structure of the crystal. We obtain an excellent receiver operating characteristic (ROC) curve with an area under the curve (AUC) of 0.90, showing that the classification model can drastically reduce computational efforts in high-throughput studies.

==> c2db-check/bands.tex <==
\begin{figure}[h!]
    \centering
    \begin{minipage}{\L\textwidth}
        \centering
        \includegraphics[width=\textwidth]{SI-benchmark-CBP/As2/plot.pdf}
        \caption{\small Phonons bands structure of As$_2$.}
        \label{fig:As2}
    \end{minipage}\hfill
%
    \begin{minipage}{\L\textwidth}
        \centering
        \includegraphics[width=\l\textwidth]{c2db-check/AsBrS.png}
        \caption{\small Phonons bands structure of AsBrS.}
        \label{fig:AsBrS}
    \end{minipage}
\end{figure}
%
%
\begin{figure}[h!]
    \centering
    \begin{minipage}{\L\textwidth}
        \centering
        \includegraphics[width=\l\textwidth]{c2db-check/AsBrSe.png}
        \caption{\small Phonons bands structure of AsBrSe.}
        \label{fig:AsBrSe}
    \end{minipage}\hfill
%
    \begin{minipage}{\L\textwidth}
        \centering
        \includegraphics[width=\l\textwidth]{c2db-check/CoTe2.png}
        \caption{\small Phonons bands structure of CoTe$_2$.}
        \label{fig:CoTe2}
    \end{minipage}
\end{figure}
%
%
\begin{figure}[h!]
    \centering
    \begin{minipage}{\L\textwidth}
        \centering
        \includegraphics[width=\l\textwidth]{c2db-check/Cr2S4.png}
        \caption{\small Phonons bands structure of Cr$_2$S$_4$.}
        \label{fig:Cr2S4}
    \end{minipage}\hfill
%
    \begin{minipage}{\L\textwidth}
        \centering
        \includegraphics[width=\l\textwidth]{c2db-check/CrS2.png}
        \caption{\small Phonons bands structure of CrS$_2$.}
        \label{fig:CrS2}
    \end{minipage}
\end{figure}
%
\clearpage%
\begin{figure}[h!]
    \centering
    \begin{minipage}{\L\textwidth}
        \centering
        \includegraphics[width=\l\textwidth]{c2db-check/F2Ge2.png}
        \caption{\small Phonons bands structure of F$_2$Ge$_2$.}
        \label{fig:F2Ge2}
    \end{minipage}\hfill
%
    \begin{minipage}{\L\textwidth}
        \centering
        \includegraphics[width=\l\textwidth]{c2db-check/F2Si2.png}
        \caption{\small Phonons bands structure of F$_2$Si$_2$.}
        \label{fig:F2Si2}
    \end{minipage}
\end{figure}
%
%
\begin{figure}[h!]
    \centering
    \begin{minipage}{\L\textwidth}
        \centering
        \includegraphics[width=\l\textwidth]{c2db-check/Fe2S4.png}
        \caption{\small Phonons bands structure of Fe$_2$S$_4$.}
        \label{fig:Fe2S4}
    \end{minipage}\hfill
%
    \begin{minipage}{\L\textwidth}
        \centering
        \includegraphics[width=\l\textwidth]{c2db-check/GeS2.png}
        \caption{\small Phonons bands structure of GeS$_2$.}
        \label{fig:GeS2}
    \end{minipage}
\end{figure}
%
%
\begin{figure}[h!]
    \centering
    \begin{minipage}{\L\textwidth}
        \centering
        \includegraphics[width=\l\textwidth]{c2db-check/GeSe2.png}
        \caption{\small Phonons bands structure of GeSe$_2$.}
        \label{fig:GeSe2}
    \end{minipage}\hfill
%
    \begin{minipage}{\L\textwidth}
        \centering
        \includegraphics[width=\l\textwidth]{c2db-check/Hf2CF2.png}
        \caption{\small Phonons bands structure of Hf$_2$CF$_2$.}
        \label{fig:Hf2CF2}
    \end{minipage}
\end{figure}
%
\clearpage%
\begin{figure}[h!]
    \centering
    \begin{minipage}{\L\textwidth}
        \centering
        \includegraphics[width=\l\textwidth]{c2db-check/HfSTe.png}
        \caption{\small Phonons bands structure of HfSTe.}
        \label{fig:HfSTe}
    \end{minipage}\hfill
%
    \begin{minipage}{\L\textwidth}
        \centering
        \includegraphics[width=\l\textwidth]{c2db-check/NbSSe.png}
        \caption{\small Phonons bands structure of NbSSe.}
        \label{fig:NbSSe}
    \end{minipage}
\end{figure}
%
%
\begin{figure}[h!]
    \centering
    \begin{minipage}{\L\textwidth}
        \centering
        \includegraphics[width=\l\textwidth]{c2db-check/PtS2.png}
        \caption{\small Phonons bands structure of PtS$_2$.}
        \label{fig:PtS2}
    \end{minipage}\hfill
%
    \begin{minipage}{\L\textwidth}
        \centering
        \includegraphics[width=\l\textwidth]{c2db-check/TaTe2.png}
        \caption{\small Phonons bands structure of TaTe$_2$.}
        \label{fig:TaTe2}
    \end{minipage}
\end{figure}
%
%
\begin{figure}[h!]
    \centering
    \begin{minipage}{\L\textwidth}
        \centering
        \includegraphics[width=\l\textwidth]{c2db-check/TiSe2.png}
        \caption{\small Phonons bands structure of TiSe$_2$.}
        \label{fig:TiSe2}
    \end{minipage}\hfill
%
    \begin{minipage}{\L\textwidth}
        \centering
        \includegraphics[width=\l\textwidth]{c2db-check/VBrCl.png}
        \caption{\small Phonons bands structure of VBrCl.}
        \label{fig:VBrCl}
    \end{minipage}
\end{figure}
%
\clearpage%
\begin{figure}[h!]
    \centering
    \begin{minipage}{\L\textwidth}
        \centering
        \includegraphics[width=\l\textwidth]{c2db-check/Y2CF2.png}
        \caption{\small Phonons bands structure of Y$_2$CF$_2$.}
        \label{fig:Y2CF2}
    \end{minipage}\hfill
%
    \begin{minipage}{\L\textwidth}
        \centering
        \includegraphics[width=\l\textwidth]{c2db-check/ZrSTe.png}
        \caption{\small Phonons bands structure of ZrSTe.}
        \label{fig:ZrSTe}
    \end{minipage}
\end{figure}
%
%

==> c2db-check/check.tex <==
\begin{figure}[h!]
    \centering
    \begin{minipage}{\L\textwidth}
        \centering
        \includegraphics[width=\l\textwidth]{c2db-check/As2}
        \caption{\small Phonons bands structure of As2}
        \label{fig:As2}
    \end{minipage}\hfill
%
    \begin{minipage}{\L\textwidth}
        \centering
        \includegraphics[width=\l\textwidth]{c2db-check/AsBrSe}
        \caption{\small Phonons bands structure of AsBrSe}
        \label{fig:AsBrSe}
    \end{minipage}
\end{figure}
%
%
\begin{figure}[h!]
    \centering
    \begin{minipage}{\L\textwidth}
        \centering
        \includegraphics[width=\l\textwidth]{c2db-check/CoTe2}
        \caption{\small Phonons bands structure of CoTe2}
        \label{fig:CoTe2}
    \end{minipage}\hfill
%
    \begin{minipage}{\L\textwidth}
        \centering
        \includegraphics[width=\l\textwidth]{c2db-check/CrS2}
        \caption{\small Phonons bands structure of CrS2}
        \label{fig:CrS2}
    \end{minipage}
\end{figure}
%
%
\begin{figure}[h!]
    \centering
    \begin{minipage}{\L\textwidth}
        \centering
        \includegraphics[width=\l\textwidth]{c2db-check/Cr2S4}
        \caption{\small Phonons bands structure of Cr2S4}
        \label{fig:Cr2S4}
    \end{minipage}\hfill
%
    \begin{minipage}{\L\textwidth}
        \centering
        \includegraphics[width=\l\textwidth]{c2db-check/Fe2S4}
        \caption{\small Phonons bands structure of Fe2S4}
        \label{fig:Fe2S4}
    \end{minipage}
\end{figure}
%
\clearpage%
\begin{figure}[h!]
    \centering
    \begin{minipage}{\L\textwidth}
        \centering
        \includegraphics[width=\l\textwidth]{c2db-check/F2Ge2}
        \caption{\small Phonons bands structure of F2Ge2}
        \label{fig:F2Ge2}
    \end{minipage}\hfill
%
    \begin{minipage}{\L\textwidth}
        \centering
        \includegraphics[width=\l\textwidth]{c2db-check/GeS2}
        \caption{\small Phonons bands structure of GeS2}
        \label{fig:GeS2}
    \end{minipage}
\end{figure}
%
%
\begin{figure}[h!]
    \centering
    \begin{minipage}{\L\textwidth}
        \centering
        \includegraphics[width=\l\textwidth]{c2db-check/GeSe2}
        \caption{\small Phonons bands structure of GeSe2}
        \label{fig:GeSe2}
    \end{minipage}\hfill
%
    \begin{minipage}{\L\textwidth}
        \centering
        \includegraphics[width=\l\textwidth]{c2db-check/HfSTe}
        \caption{\small Phonons bands structure of HfSTe}
        \label{fig:HfSTe}
    \end{minipage}
\end{figure}
%
%
\begin{figure}[h!]
    \centering
    \begin{minipage}{\L\textwidth}
        \centering
        \includegraphics[width=\l\textwidth]{c2db-check/AsBrS}
        \caption{\small Phonons bands structure of AsBrS}
        \label{fig:AsBrS}
    \end{minipage}\hfill
%
    \begin{minipage}{\L\textwidth}
        \centering
        \includegraphics[width=\l\textwidth]{c2db-check/Hf2CF2}
        \caption{\small Phonons bands structure of Hf2CF2}
        \label{fig:Hf2CF2}
    \end{minipage}
\end{figure}
%
\clearpage%
\begin{figure}[h!]
    \centering
    \begin{minipage}{\L\textwidth}
        \centering
        \includegraphics[width=\l\textwidth]{c2db-check/Y2CF2}
        \caption{\small Phonons bands structure of Y2CF2}
        \label{fig:Y2CF2}
    \end{minipage}\hfill
%
    \begin{minipage}{\L\textwidth}
        \centering
        \includegraphics[width=\l\textwidth]{c2db-check/FeTe2}
        \caption{\small Phonons bands structure of FeTe2}
        \label{fig:FeTe2}
    \end{minipage}
\end{figure}
%
%
\begin{figure}[h!]
    \centering
    \begin{minipage}{\L\textwidth}
        \centering
        \includegraphics[width=\l\textwidth]{c2db-check/NbSSe}
        \caption{\small Phonons bands structure of NbSSe}
        \label{fig:NbSSe}
    \end{minipage}\hfill
%
    \begin{minipage}{\L\textwidth}
        \centering
        \includegraphics[width=\l\textwidth]{c2db-check/PtS2}
        \caption{\small Phonons bands structure of PtS2}
        \label{fig:PtS2}
    \end{minipage}
\end{figure}
%
%
\begin{figure}[h!]
    \centering
    \begin{minipage}{\L\textwidth}
        \centering
        \includegraphics[width=\l\textwidth]{c2db-check/F2Si2}
        \caption{\small Phonons bands structure of F2Si2}
        \label{fig:F2Si2}
    \end{minipage}\hfill
%
    \begin{minipage}{\L\textwidth}
        \centering
        \includegraphics[width=\l\textwidth]{c2db-check/TaTe2}
        \caption{\small Phonons bands structure of TaTe2}
        \label{fig:TaTe2}
    \end{minipage}
\end{figure}
%
\clearpage%
\begin{figure}[h!]
    \centering
    \begin{minipage}{\L\textwidth}
        \centering
        \includegraphics[width=\l\textwidth]{c2db-check/TiSe2}
        \caption{\small Phonons bands structure of TiSe2}
        \label{fig:TiSe2}
    \end{minipage}\hfill
%
    \begin{minipage}{\L\textwidth}
        \centering
        \includegraphics[width=\l\textwidth]{c2db-check/VBrCl}
        \caption{\small Phonons bands structure of VBrCl}
        \label{fig:VBrCl}
    \end{minipage}
\end{figure}
%

==> tables/1-data.tex <==
\begin{tabular}{lllllllll}
\hline
Material & 
\multicolumn{2}{c}{Hull (eV/atom)} &
\multicolumn{2}{c}{Hessian (eV/\AA^2)} &
\multicolumn{2}{c}{E$_\textup{gap}^{\text{PBE}}$ (eV)} &
\multicolumn{2}{c}{$D(E_F)$} &%(states/(eV pc))
\\
 & before & after & before & after & before & after & before & after \\ \hline
\\
Ag$_{2}$Br$_{4}$ & 0.14 & -0.0 & -3.1 & -0.3 & 0.0 & 0.0 & -1 \\
Ag$_{2}$Br$_{4}$ & 0.04 & -0.0 & -1.0 & 0.04 & 0.0 & 0.0 & 6.76 \\
Ag$_{2}$Br$_{4}$ & 0.05 & 0.00 & -0.9 & -0.0 & 0.0 & 0.0 & 2.70 \\
Ag$_{2}$Cl$_{4}$ & 0.04 & -0.0 & -2.5 & 0.06 & 0.0 & 0.0 & 8.49 \\
As$_{2}$Cl$_{2}$Te$_{2}$ & 0.18 & 0.01 & -0.2 & 0.25 & 1.28 & 1.48 & 0.0 \\
Co$_{2}$Se$_{4}$ & 0.05 & 0.03 & -4.8 & 0.09 & 0.0 & 0.12 & 1.38 \\
Co$_{4}$P$_{4}$S$_{12}$ & 0.07 & 0.05 & -3.4 & -0.2 & 0.0 & 0.09 & 1.68 \\
Cr$_{2}$Br$_{2}$Cl$_{2}$ & 0.09 & 0.06 & -0.9 & 0.14 & 0.0 & 0.64 & 3.67 \\
Cr$_{2}$Br$_{4}$ & 0.07 & 0.06 & -0.5 & 0.06 & 0.0 & 0.49 & 3.91 \\
Cr$_{2}$Cl$_{4}$ & 0.10 & 0.05 & -1.8 & 0.14 & 0.0 & 0.75 & 4.91 \\
Cr$_{2}$I$_{4}$ & 0.17 & 0.11 & -3.9 & -0.0 & 0.0 & 1.07 & -1 \\
Cr$_{2}$S$_{2}$Se$_{2}$ & 0.14 & 0.08 & -9.7 & 0.71 & 0.0 & 0.0 & 0.26 \\
Cr$_{2}$S$_{4}$ & 0.11 & 0.10 & -15. & 0.73 & 0.0 & 0.0 & 0.26 \\
Cr$_{2}$Se$_{4}$ & 0.13 & 0.05 & -12. & 0.77 & 0.0 & 0.0 & 0.31 \\
Cr$_{4}$P$_{4}$S$_{12}$ & 0.05 & 0.03 & -3.1 & 999 & 0.0 & 0.34 & -1 \\
Hf$_{2}$Br$_{2}$Cl$_{2}$ & 0.04 & 0.03 & -9.6 & 0.39 & 0.0 & 0.81 & 0.46 \\
Hf$_{2}$Br$_{2}$I$_{2}$ & 0.12 & 0.05 & -10. & 0.38 & 0.0 & 0.73 & 0.57 \\
Hf$_{2}$Br$_{4}$ & -0.0 & -0.0 & -10. & 0.40 & 0.0 & 0.84 & 0.49 \\
Hf$_{2}$Cl$_{4}$ & 0.12 & 0.04 & -8.5 & 0.38 & 0.0 & 0.85 & 0.46 \\
Mn$_{2}$S$_{4}$ & -0.0 & 0.11 & -2.4 & -9.2 & 0.0 & 0.0 & 3.75 \\
Mn$_{2}$Se$_{4}$ & -0.0 & 0.12 & -3.9 & -7.2 & 0.0 & 0.0 & 2.53 \\
Mo$_{2}$Se$_{2}$Te$_{2}$ & 0.19 & 0.07 & -10. & 0.68 & 0.0 & 0.0 & 0.0 \\
Mo$_{2}$Te$_{4}$ & 0.17 & 0.01 & -13. & 0.66 & 0.0 & 0.0 & 0.41 \\
Nb$_{2}$Cl$_{4}$ & 0.19 & 0.11 & -3.8 & -2.6 & 0.0 & 0.0 & 0.63 \\
Nb$_{2}$S$_{2}$Se$_{2}$ & -0.0 & -0.0 & -2.1 & -1.2 & 0.0 & 0.0 & 1.40 \\
Nb$_{2}$S$_{2}$Te$_{2}$ & 0.07 & 0.06 & -4.7 & -2.6 & 0.0 & 0.0 & 2.11 \\
Nb$_{2}$Se$_{2}$Te$_{2}$ & 0.01 & 0.00 & -2.3 & -1.6 & 0.0 & 0.0 & 1.79 \\
Pd$_{2}$I$_{4}$ & 0.16 & 0.02 & -0.5 & 0.11 & 0.0 & 0.59 & 2.66 \\
Re$_{2}$Te$_{4}$ & 0.18 & 0.17 & -3.0 & -2.4 & 0.0 & 0.0 & 1.01 \\
Rh$_{2}$O$_{4}$ & 0.15 & 0.14 & -2.1 & 0.65 & 0.0 & 0.0 & 1.82 \\
Ta$_{2}$S$_{2}$Te$_{2}$ & 0.04 & 0.03 & -5.1 & -3.4 & 0.0 & 0.0 & 1.91 \\
Ta$_{2}$S$_{2}$Te$_{2}$ & 0.04 & 0.03 & -2.2 & -3.4 & 0.0 & 0.0 & -1 \\
Ta$_{2}$Se$_{2}$Te$_{2}$ & 0.03 & 0.02 & -2.6 & -1.6 & 0.0 & 0.0 & 1.82 \\
Ti$_{2}$Br$_{2}$Cl$_{2}$ & 0.05 & -0.0 & -9.1 & 0.51 & 0.0 & 0.29 & 1.14 \\
Ti$_{2}$Cl$_{4}$ & 0.02 & -0.0 & -9.9 & 0.52 & 0.0 & 0.32 & 1.00 \\
Ti$_{6}$F$_{4}$N$_{4}$ & -0.0 & 0.07 & -4.2 & -2.0 & 0.0 & 0.0 & 5.33 \\
Ti$_{6}$F$_{4}$N$_{4}$ & -0.0 & 0.07 & -4.5 & -2.0 & -1 & 0.0 & -1 \\
V$_{2}$O$_{4}$ & 0.12 & 0.10 & -3.5 & -3.1 & 0.0 & 0.0 & 2.05 \\
Zr$_{2}$Br$_{2}$Cl$_{2}$ & 0.08 & 0.02 & -8.0 & 0.39 & 0.0 & 0.59 & 0.51 \\
Zr$_{2}$Br$_{2}$I$_{2}$ & 0.12 & 0.01 & -8.8 & 0.38 & 0.0 & 0.48 & 0.62 \\
Zr$_{2}$Br$_{4}$ & 0.06 & -0.0 & -8.6 & 0.47 & 0.0 & 0.59 & 0.54 \\
Zr$_{2}$Cl$_{2}$I$_{2}$ & 0.18 & 0.07 & -8.6 & 0.26 & 0.0 & 0.47 & 0.64 \\
Zr$_{2}$Cl$_{4}$ & 0.09 & 0.02 & -7.1 & 0.46 & 0.0 & 0.59 & 0.53 \\
Zr$_{2}$I$_{4}$ & 0.13 & -0.0 & -8.5 & 0.47 & 0.0 & 0.42 & 0.73 \\
\hline
\bottomrule
\end{tabular}

==> tables/2-data.tex <==
\begin{tabular}{llllllllll}
\toprule
Material & Prototype & 
\multicolumn{2}{c}{Hull (eV/atom)} &
\multicolumn{2}{c}{Hessian (eV/\AA^2)} &
\multicolumn{2}{c}{E$_\textup{gap}^{\text{PBE}}$ (eV)} &
\multicolumn{2}{c}{$D(E_F)$} &%(states/(eV pc))
\\
 & & before & after & before & after & before & after & before & after \\
\\
NbCl2 & CdI2 & 0.19 & 0.19 & -3.8 & -2.6 & 0.0 & 0.0 & 0.63 & 0.63 \\
NbS2 & MoS2 & 0.00 & 0.00 & -1.4 & 0.02 & 0.0 & 0.0 & 1.30 & 1.30 \\
NbSe2 & MoS2 & 0.00 & 0.00 & -0.1 & 0.00 & 0.0 & 0.0 & 1.34 & 1.34 \\
NbSeTe & MoSSe & 0.01 & 0.01 & -2.3 & 0.00 & 0.0 & 0.0 & 1.79 & 1.79 \\
NbSSe & MoSSe & -0.0 & -0.0 & -2.1 & 0.00 & 0.0 & 0.0 & 1.40 & 1.40 \\
NbSTe & MoSSe & 0.07 & 0.07 & -4.7 & 0.01 & 0.0 & 0.0 & 2.11 & 2.11 \\
Ni2O2 & GaS & 0.04 & 0.04 & -0.1 & -1.3 & 0.0 & 0.0 & 4.34 & 4.34 \\
PdI2 & CdI2 & 0.16 & 0.16 & -0.5 & 0.00 & 0.0 & 0.0 & 2.66 & 2.66 \\
ReTe2 & MoS2 & 0.18 & 0.18 & -3.0 & -5.0 & 0.0 & 0.0 & 1.01 & 1.01 \\
Rh2I2 & CH & 0.16 & 0.16 & -0.3 & -0.0 & 0.0 & 0.0 & 1.49 & 1.49 \\
Rh2Se2 & GaSe & 0.19 & 0.19 & -0.4 & -0.5 & 0.0 & 0.0 & 1.65 & 1.65 \\
RhI2 & CdI2 & -0.1 & -0.1 & -0.6 & 0.00 & 0.0 & 0.0 & 2.01 & 2.01 \\
RhO2 & CdI2 & 0.15 & 0.15 & -2.1 & 0.01 & 0.0 & 0.0 & 1.82 & 1.82 \\
RhTe2 & CdI2 & 0.11 & 0.11 & -1.8 & 0.01 & 0.0 & 0.0 & 0.97 & 0.97 \\
Ru2P2S6 & MnPSe3 & 0.17 & 0.17 & -1.1 & 0.00 & 0.32 & 0.32 & 0.0 & 0.0 \\
Sc2I6 & BiI3 & -0.2 & -0.2 & -0.2 &  - & 1.85 & 1.85 & 0.0 & 0.0 \\
TaSeTe & MoSSe & 0.03 & 0.03 & -2.6 & -0.1 & 0.0 & 0.0 & 1.82 & 1.82 \\
TaSSe & MoSSe & 0.00 & 0.00 & -1.2 & 0.00 & 0.0 & 0.0 & 1.25 & 1.25 \\
TaSTe & MoSSe & 0.04 & 0.04 & -2.2 & -0.4 & 0.0 & 0.0 & 0 & 0 \\
TaSTe & MoSSe & 0.04 & 0.04 & -5.1 & -0.4 & 0.0 & 0.0 & 1.91 & 1.91 \\
TaTe2 & MoS2 & 0.04 & 0.04 & -0.5 & 0.00 & 0.0 & 0.0 & 1.94 & 1.94 \\
Ti2P2Se6 & MnPSe3 & 0.16 & 0.16 & -1.4 & 0.06 & 0.0 & 0.0 & 2.54 & 2.54 \\
Ti2P2Se6 & MnPSe3 & 0.16 & 0.16 & -1.4 &  - & 0.0 & 0.0 & 31.8 & 31.8 \\
Ti3F2N2 & Ti3C2O2 & -0.0 & -0.0 & -4.2 & -1.5 & 0.0 & 0.0 & 5.33 & 5.33 \\
Ti3F2N2 & Ti3C2O2 & -0.0 & -0.0 & -4.5 & -1.5 & 0 & 0 & 0 & 0 \\
Ti3H2N2O2 & Ti3C2H2O2 & 0.08 & 0.08 & -0.5 & -0.0 & 0.0 & 0.0 & 3.12 & 3.12 \\
TiBr2 & CdI2 & 0.01 & 0.01 & -0.6 & 0.01 & 0.0 & 0.0 & 2.30 & 2.30 \\
TiBrCl & BiTeI & 0.05 & 0.05 & -9.1 & 1.82 & 0.0 & 0.0 & 1.14 & 1.14 \\
TiCl2 & CdI2 & 0.02 & 0.02 & -9.9 & 0.00 & 0.0 & 0.0 & 1.00 & 1.00 \\
TiO2 & CdI2 & 0.13 & 0.13 & -1.9 & 0.01 & 2.70 & 2.70 & 0.0 & 0.0 \\
TiS2 & CdI2 & -0.0 & -0.0 & -1.5 & -0.0 & 0.0 & 0.0 & 0.07 & 0.07 \\
TiS2 & MoS2 & 0.14 & 0.14 & -0.5 & -0.1 & 0.73 & 0.73 & 0.0 & 0.0 \\
TiSe2 & CdI2 & -0.0 & -0.0 & -1.3 & 0.00 & 0.0 & 0.0 & 0.58 & 0.58 \\
TiSSe & BiTeI & -0.0 & -0.0 & -0.5 & 0.00 & 0.0 & 0.0 & 0.09 & 0.09 \\
V2NO2 & Ti2CO2 & 0.14 & 0.14 & -0.6 & -0.0 & 0.0 & 0.0 & 3.26 & 3.26 \\
VO2 & CdI2 & 0.12 & 0.12 & -3.5 & -0.4 & 0.0 & 0.0 & 2.05 & 2.05 \\
VTe2 & CdI2 & 0.01 & 0.01 & -1.3 & 0.02 & 0.0 & 0.0 & 1.48 & 1.48 \\
YBr2 & CdI2 & -0.1 & -0.1 & -1.0 & 0.00 & 0.0 & 0.0 & 0.78 & 0.78 \\
YI2 & CdI2 & 0.04 & 0.04 & -0.4 & -0.1 & 0.0 & 0.0 & 0.88 & 0.88 \\
ZrBr2 & CdI2 & 0.06 & 0.06 & -8.6 & 0.01 & 0.0 & 0.0 & 0.54 & 0.54 \\
ZrBrCl & BiTeI & 0.08 & 0.08 & -8.0 & 0.01 & 0.0 & 0.0 & 0.51 & 0.51 \\
ZrBrI & BiTeI & 0.12 & 0.12 & -8.8 & 0.01 & 0.0 & 0.0 & 0.62 & 0.62 \\
ZrCl2 & CdI2 & 0.09 & 0.09 & -7.1 & 0.00 & 0.0 & 0.0 & 0.53 & 0.53 \\
ZrClI & BiTeI & 0.18 & 0.18 & -8.6 & 0.00 & 0.0 & 0.0 & 0.64 & 0.64 \\
ZrI2 & CdI2 & 0.13 & 0.13 & -8.5 & 0.00 & 0.0 & 0.0 & 0.73 & 0.73 \\
ZrS2 & MoS2 & 0.18 & 0.18 & -0.9 & 0.00 & 0.96 & 0.96 & 0.0 & 0.0 \\
\midrule
\bottomrule
\end{tabular}

==> tables/ehull.tex <==
\begin{tabular}{lllllllll}
	%\toprule
	\hline
	id &
	Material & Crystal type &
	\multicolumn{2}{c}{Hull (eV/atom)} &
	\multicolumn{2}{c}{Hessian (eV/AA)} &
	\multicolumn{2}{c}{$\varepsilon_\textup{gap}^{\text{\tiny PBE}}$ (eV)}
	\\
	& & & before & after & before & after & before & after \\ \hline
	%\midrule
1 & Ag$_{2}$Cl$_{4}$ & AB2-1-a &  0.04 & -0.0 & -2.5 & 0.06 & 0.0 & 0.0 \\
2 & In$_{8}$Se$_{8}$ & AB-6-ab & -0.0 & -0.0 & -0.2 & 0.01 & 1.4 & 1.39 \\
3 & Nb$_{4}$Te$_{8}$ & AB2-1-a & -0.0 & -0.0 & -0.3 & 0.51 & 0.0 & 0.0 \\
4 & Rh$_{2}$I$_{4}$ & AB2-1-a & -0.1 & 0.16 & -0.6 & 0.03 & 0.0 & 0.0 \\
5 & Sc$_{4}$I$_{12}$ & AB3-1-a & -0.28 & -0.0 & -0.2 & 0.01 & 1.84 & 1.84 \\
6 & Ti$_{2}$Br$_{2}$Cl$_{2}$ & ABC-1-a & 0.05 & -0.0 & -9.1 & 0.51 & 0.0 & 0.29 \\
7 & Ti$_{2}$Cl$_{4}$ & AB2-2-i & 0.02 & -0.0 & -9.9 & 0.52 & 0.0 & 0.32 \\
8 & Zr$_{2}$Br$_{4}$ & AB2-2-i & 0.06 & -0.0 & -8.6 & 0.47 & 0.0 & 0.59 \\
9 & Zr$_{2}$I$_{4}$ & AB2-2-i & 0.13 & -0.0 & -8.5 & 0.47 & 0.0 & 0.42 \\
	\hline
%	\bottomrule
\end{tabular}

==> tables/old-stable.tex <==
\begin{tabular}{llllllllll}
	\hline
	id &
	Material & Prototype & Spacegroup &
	\multicolumn{2}{c}{Hull (eV/atom)} &
	\multicolumn{2}{c}{Hessian (eV/AA)} &
	\multicolumn{2}{c}{E$_\textup{gap}^{\text{PBE}}$ (eV)}
	\\
	& & & & before & after & before & after & before & after \\ \hline
	\\
1 & Ag$_{2}$Br$_{4}$ & CdI2 & P1 & 0.04 & -0.0 & -1.0 & 0.04 & 0.0 & 0.0 \\
2 & Ag$_{2}$Cl$_{4}$ & CdI2 & P1 & 0.04 & -0.0 & -2.5 & 0.06 & 0.0 & 0.0 \\
3 & As$_{2}$Cl$_{2}$Te$_{2}$ & MoSSe & P1 & 0.18 & 0.01 & -0.2 & 0.25 & 1.28 & 1.48 \\
4 & Cd$_{4}$Br$_{4}$ & - & P1 & - & 0.06 & -1.0 & 0.03 & - & 1.28 \\
5 & Cd$_{4}$Cl$_{4}$ & - & P1 & - & 0.04 & -0.7 & 0.17 & - & 1.67 \\
6 & Co$_{2}$Se$_{4}$ & CdI2 & P-1 & 0.05 & 0.03 & -4.8 & 0.09 & 0.0 & 0.12 \\
7 & Cr$_{2}$Br$_{2}$Cl$_{2}$ & BiTeI & P1 & 0.09 & 0.06 & -0.9 & 0.14 & 0.0 & 0.64 \\
8 & Cr$_{2}$Br$_{4}$ & CdI2 & P1 & 0.07 & 0.06 & -0.5 & 0.06 & 0.0 & 0.49 \\
9 & Cr$_{2}$Cl$_{4}$ & CdI2 & P1 & 0.10 & 0.05 & -1.8 & 0.14 & 0.0 & 0.75 \\
10 & Cr$_{2}$S$_{2}$Se$_{2}$ & BiTeI & P1 & 0.14 & 0.08 & -9.7 & 0.71 & 0.0 & 0.0 \\
11 & Cr$_{2}$S$_{4}$ & CdI2 & P-1 & 0.11 & 0.10 & -15. & 0.73 & 0.0 & 0.0 \\
12 & Cr$_{2}$Se$_{4}$ & CdI2 & P-1 & 0.13 & 0.05 & -12. & 0.77 & 0.0 & 0.0 \\
13 & Cr$_{2}$Te$_{4}$ & - & P1 & - & 0.01 & -1.9 & 0.08 & - & 0.0 \\
14 & Cr$_{4}$P$_{4}$S$_{12}$ & MnPSe3 & P-1 & 0.05 & 0.03 & -3.1 & - & 0.0 & 0.34 \\
15 & Fe$_{2}$Te$_{4}$ & - & P1 & - & - & -1.9 & - & - & - \\
16 & Fe$_{4}$P$_{4}$Se$_{12}$ & - & P1 & - & 0.12 & -1.0 & 0.04 & - & 0.12 \\
17 & Fe$_{4}$Se$_{8}$ & - & P1 & - & - & -0.5 & 0.38 & - & - \\
18 & Fe$_{8}$P$_{8}$Se$_{24}$ & - & P1 & - & 0.12 & -1.0 & - & - & 0.12 \\
19 & Hf$_{2}$Br$_{2}$Cl$_{2}$ & BiTeI & P1 & 0.04 & 0.03 & -9.6 & 0.39 & 0.0 & 0.81 \\
20 & Hf$_{2}$Br$_{2}$I$_{2}$ & BiTeI & P1 & 0.12 & 0.05 & -10. & 0.38 & 0.0 & 0.73 \\
21 & Hf$_{2}$Br$_{4}$ & CdI2 & P-1 & -0.0 & -0.0 & -10. & 0.40 & 0.0 & 0.84 \\
22 & Hf$_{2}$Cl$_{4}$ & CdI2 & P-1 & 0.12 & 0.04 & -8.5 & 0.38 & 0.0 & 0.85 \\
23 & Hg$_{4}$Se$_{4}$ & - & P1 & - & 0.04 & -0.8 & 0.04 & - & 0.36 \\
24 & Hg$_{4}$Te$_{4}$ & - & P1 & - & 0.04 & -0.6 & 0.03 & - & 0.37 \\
25 & In$_{4}$Te$_{4}$ & - & P1 & - & 0.09 & -0.4 & 0.23 & - & 0.0 \\
26 & In$_{8}$Br$_{8}$Se$_{8}$ & - & P-1 & - & 0.02 & -0.5 & 0.04 & - & 1.22 \\
27 & In$_{8}$Se$_{8}$ & - & Pm & - & -0.0 & -0.2 & 0.01 & - & 1.39 \\
28 & Mo$_{2}$Se$_{2}$Te$_{2}$ & BiTeI & P1 & 0.19 & 0.07 & -10. & 0.68 & 0.0 & 0.0 \\
29 & Mo$_{2}$Te$_{4}$ & CdI2 & P-1 & 0.17 & 0.01 & -13. & 0.66 & 0.0 & 0.0 \\
30 & Nb$_{2}$S$_{4}$ & - & Pm & - & -0.0 & -1.4 & 0.05 & - & 0.0 \\
31 & Nb$_{4}$Te$_{8}$ & - & P1 & - & - & -0.3 & 0.51 & - & - \\
32 & Pd$_{2}$I$_{4}$ & CdI2 & P1 & 0.16 & 0.02 & -0.5 & 0.11 & 0.0 & 0.59 \\
33 & Rh$_{2}$I$_{4}$ & - & P1 & - & 0.16 & -0.6 & 0.03 & - & 0.0 \\
34 & Rh$_{2}$O$_{4}$ & CdI2 & P-1 & 0.15 & 0.14 & -2.1 & 0.65 & 0.0 & 0.0 \\
35 & Rh$_{2}$Te$_{4}$ & - & P1 & - & 0.07 & -1.8 & 0.35 & - & 0.12 \\
36 & Sc$_{4}$I$_{12}$ & - & P1 & - & -0.0 & -0.2 & 0.01 & - & 1.84 \\
37 & Ti$_{2}$Br$_{2}$Cl$_{2}$ & BiTeI & P1 & 0.05 & -0.0 & -9.1 & 0.51 & 0.0 & 0.29 \\
38 & Ti$_{2}$Br$_{4}$ & - & P1 & - & 0.04 & -0.6 & 0.30 & - & 0.11 \\
39 & Ti$_{2}$Cl$_{4}$ & CdI2 & P-1 & 0.02 & -0.0 & -9.9 & 0.52 & 0.0 & 0.32 \\
40 & Ti$_{2}$O$_{4}$ & - & Pm & - & 0.12 & -1.9 & 0.47 & - & 2.85 \\
41 & Ti$_{2}$S$_{4}$ & - & P2$_1$ & - & 0.13 & -0.5 & 0.00 & - & 0.79 \\
42 & Ti$_{4}$P$_{4}$Se$_{12}$ & - & P1 & - & 0.12 & -1.4 & - & - & 0.0 \\
43 & V$_{2}$Te$_{4}$ & - & Pm & - & 0.00 & -1.3 & 0.38 & - & 0.0 \\
44 & Zr$_{2}$Br$_{2}$Cl$_{2}$ & BiTeI & P1 & 0.08 & 0.02 & -8.0 & 0.39 & 0.0 & 0.59 \\
45 & Zr$_{2}$Br$_{2}$I$_{2}$ & BiTeI & P1 & 0.12 & 0.01 & -8.8 & 0.38 & 0.0 & 0.48 \\
46 & Zr$_{2}$Br$_{4}$ & CdI2 & P-1 & 0.06 & -0.0 & -8.6 & 0.47 & 0.0 & 0.59 \\
47 & Zr$_{2}$Cl$_{2}$I$_{2}$ & BiTeI & P1 & 0.18 & 0.07 & -8.6 & 0.26 & 0.0 & 0.47 \\
48 & Zr$_{2}$Cl$_{4}$ & CdI2 & P-1 & 0.09 & 0.02 & -7.1 & 0.46 & 0.0 & 0.59 \\
49 & Zr$_{2}$I$_{4}$ & CdI2 & P-1 & 0.13 & -0.0 & -8.5 & 0.47 & 0.0 & 0.42 \\
50 & Zr$_{2}$S$_{4}$ & - & P2$_1$ & - & 0.18 & -0.9 & 0.15 & - & 1.12 \\
	\hline
	\bottomrule
\end{tabular}
